Adapting Definition Modeling for New Languages: A Case Study on Belarusian

Definition modeling, the task of generating new definitions for words in context, holds great prospect as a means to assist the work of lexicographers in documenting a broader variety of lects and languages, yet much remains to be done in order to assess how we can leverage pre-existing models for as-of-yet unsupported languages. In this work, we focus on adapting existing models to Belarusian, for which we propose a novel dataset of 43,150 definitions. Our experiments demonstrate that adapting a definition modeling systems requires minimal amounts of data, but that there currently are gaps in what automatic metrics do capture.

==> tables/average_manual.tex <==
\begin{table}[ht]
\toprule
\begin{tabular}{l *{6}{S}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{6}{c}{\textbf{Data}} \\
\cmidrule(lr){2-7}
 & {\textbf{0\%}} & {\textbf{1\%}} & {\textbf{3\%}} & {\textbf{10\%}} & {\textbf{31\%}} & {\textbf{100\%}} \\
\midrule
Fluency           & 0.026 & 0.756 & 0.833 & 0.814 & 0.800 & 0.851 \\
Informativeness   & 0.520 & 0.373 & 0.355 & 0.497 & 0.583 & 0.636 \\
\bottomrule
\end{tabular}
\end{table}
